Periodic leaf-wise intersection points from Lagrangians

We investigate leaf-wise intersection points on hypersurfaces of contact type in monotone symplectic manifolds. We show that monotone Floer-essential Lagrangians detect periodic leaf-wise intersection points in hypersurfaces of contact type whose Reeb flow is Zoll. Examples include the prequantization bundles appearing in monotone toric negative line bundles. Generalizing, we prove the existence of leaf-wise intersection points for certain annulus subbundles in weak+-monotone negative line bundles, not necessarily toric. The proofs combine reduced symplectic cohomology with the original methods employed by Albers-Frauenfelder to prove global existence results of this kind.

==> Leafwise copy/ssv_artmac.tex <==

%%		PREAMBLE
%%
%%            PAGE LAYOUT
%%
%\setlength{\oddsidemargin}{31 pt}
%\setlength{\evensidemargin}{90.755 pt}
%\setlength{\topmargin}{28 pt}
%\setlength{\topmargin}{-5 pt}
%\setlength{\headheight}{12 pt}
%\setlength{\headsep}{20 pt}
%\setlength{\textheight}{522 pt}          % For 12 pt
%\setlength{\textheight}{620 pt}           % For 10 pt
%\setlength{\textheight}{48\baselineskip} % For 10 pt
%\setlength{\textwidth}{426 pt}
%\setlength{\footskip}{36 pt}
%\setlength{\parindent}{0.5 in}
%
%		PAGE STYLE
%
%\setlength{\oddsidemargin}{0.5 in}
%\setlength{\evensidemargin}{0.5 in}
%%\setlength{\oddsidemargin}{0.25 in}
%%\setlength{\evensidemargin}{0.25 in}
%%\setlength{\marginparsep}{0.125 in}
%%\setlength{\marginparwidth}{1.25in}
%\setlength{\marginparwidth}{71 pt}
%\setlength{\marginparsep}{7 pt}
%\setlength{\marginparpush}{5pt}
%%\normalsize
%\setlength{\textheight}{50\baselineskip}
%%\setlength{\textheight}{52\baselineskip}
%\setlength{\textwidth}{5.5 in}
%%\setlength{\textwidth}{6in}
%\setlength{\topmargin}{0 in}
%%\setlength{\topmargin}{-0.5 in}
%\setlength{\headheight}{12 pt}
%\setlength{\headsep}{25 pt}
%\setlength{\footskip}{36 pt}
%\setlength{\parindent}{20 pt}
%%\setlength{\topskip}{0.5 in}
%%\setlength{\footheight}{0.25 in}
%%\setlength{\baselineskip}{12pt}
%
%		HEADER AND FOOTER
%
%\pagestyle{headings}
%\pagestyle{fancyplain}
%\addtolength{\headwidth}{\marginparsep}
%\addtolength{\headwidth}{\marginparwidth}
%  Remember section number and title
\renewcommand{\sectionmark}[1]{\markboth{\thesection\ #1}{\thesection\ #1}}
%  Remember subsection number and title
\renewcommand{\subsectionmark}[1]{\markright{\thesection.\thesubsection\ #1}}
\setlength{\headrulewidth}{0.4pt}
\setlength{\plainheadrulewidth}{0pt}
\setlength{\plainfootrulewidth}{0.8pt}
%             Left Head---even & odd pages, plain & normal variations
\lhead%
  [\fancyplain{}{\bfseries\thepage}]{\fancyplain{}{\bfseries\rightmark}}
%             Centre Head---even & odd pages, plain & normal variations
\chead[\fancyplain{}{}]{\fancyplain{}{}}
%             Right Head---even & odd pages, plain & normal variations
\rhead%
  [\fancyplain{}{\bfseries\leftmark}]{\fancyplain{}{\bfseries\thepage}}
%             Centre Foot
\cfoot{}
%\cfoot{\fancyplain{\emph{SK,SSV, 06.08.2007}}{}}
%
\pagenumbering{arabic}
%
%		FOOTER
%
\setlength{\footnotesep}{12pt}
%
%%
%%            NEWCOMMAND DEFINITIONS---AMS LATEX FORMAT & EULER FONTS NEEDED
%%
\newcommand{\colim}{\text{colim}}
\newcommand{\attention}{\marginpar{$\longleftrightarrow$}}
\newcommand{\Bigo}{\mathscr{O}}
\let\binomial=\binom
\newcommand{\Bn}{ \binary^n }
\newcommand{\bE}{\operatorname{\mathbf{E}}}
\newcommand{\binary}{\mathbb{B}}
\newcommand{\boldone}{\boldsymbol{1}}  % same as \mathbf{1}
\newcommand{\boldzero}{\boldsymbol{0}} % same as \mathbf{0}
\newcommand{\card}{\operatorname{card}}
\let\choice=\binom
\newcommand{\cl}{\operatorname{cl}}
\let\combination=\binom
\newcommand{\complex}{\mathbb{C}}
\newcommand{\composition}{ \circ }
\newcommand{\Complement}{{\scriptscriptstyle\complement}}
\newcommand{\condition}[1]{\qquad #1}
\def\Cov{\mathop{\text{\normalfont\upshape Cov}}\nolimits} 
\newcommand{\cov}{\Cov}
  % prevents \it in theorems
%\let\defn=\triangleq
\newcommand{\defn}{ := }
\newcommand{\del}{ \delta }
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\efrac}[2]{{\scriptscriptstyle\frac{#1}{#2}}}
\newcommand{\eps}{ \epsilon }
\let\expectation=\bE
\let\frak=\mathfrak
\newcommand{\fracwithdelims}[4]{\left#1 \frac{#3}{#4} \right#2}
\renewcommand{\gcd}{\operatorname{gcd}}
\newcommand{\graphdeg}{\operatorname{deg}}
\let\gtsim=\gtrsim
\newcommand{\half}{\frac{1}{2}}
\newcommand{\hilbert}{\mathbb{H}}
\newcommand{\inae}{\overset{\textit{\tiny a.e.}}\rightarrow}
\newcommand{\Index}[1]{#1\index{#1}}
\newcommand{\indist}{\overset{\textit{\tiny d}}\rightarrow}
\newcommand{\inprob}{\overset{\textit{\tiny p}}\rightarrow}
\newcommand{\invague}{\overset{\textit{\tiny v}}\rightarrow}
\newcommand{\inweak}{\overset{\textit{\tiny w}}\rightarrow}
\newcommand{\integer}{\mathbb{Z}}
\let\ltsim=\lesssim
\newcommand{\marginalnote}[1]{\marginpar{\footnotesize\emph{#1}}}
\newcommand{\Median}{\operatorname{\text{\normalfont\upshape Median}}}
\newcommand{\osc}{\operatorname{\text{\normalfont\upshape osc}}}
\renewcommand{\emptyset}{\mathop{\varnothing}} % Redefines \emptyset
%\def\Paren#1{{\left({#1}\right)}}
\newcommand{\per}{\operatorname{per}}
\newcommand{\posinteger}{\mathbb{N}}
\newcommand{\prob}{\operatorname{\mathbf{P}}}
\newcommand{\qed}{\mbox{\hfill$\square$}}
\newcommand{\rational}{\mathbb{Q}}
\let\refeq=\eqref                              % \eqref defined in mathref.sty
\newcommand{\resetcounters}{%                  % Reset counters
    \setcounter{assertion}{0}
    \setcounter{conjecture}{0}
    \setcounter{corollary}{0}
    \setcounter{counterexample}{0}
    \setcounter{definition}{0}
    \setcounter{example}{0}
    \setcounter{fact}{0}
    \setcounter{lemma}{0}
    \setcounter{proposition}{0}
    \setcounter{slogan}{0}
    \setcounter{theorem}{0}
    \setcounter{remark}{0}
  }
\newcommand{\real}{\mathbb{R}}
\def\rect{\mathop{\text{\normalfont\upshape rect}}\nolimits} 
  % prevents \it in thms
\newcommand{\Rn}{ \real^n }
%\newcommand{\setcomplement}[1]{{#1}^{\text{c}}}
\newcommand{\setcomplement}[1]{{#1}^{\Complement}}
\def\sgn{\mathop{\text{\normalfont\upshape sgn}}\nolimits} 
  % prevents \it in thms
\def\sinc{\mathop{\text{\normalfont\upshape sinc}}\nolimits} 
  % prevents \it in thms
\newcommand{\smallo}{\mathfrak{o}}
\newcommand{\symmetricdifference}{\mathop{\vartriangle}}
\newcommand{\tfracwithdelims}[4]{\bigl#1\tfrac{#3}{#4}\bigr#2}
\def\Var{\mathop{\text{\normalfont\upshape Var}}\nolimits} 
\newcommand{\var}{\Var}
\newcommand{\Vol}{\operatorname{Vol}}

\newcommand{\bigslant}[2]{{\raisebox{.2em}{$#1$}\left/\raisebox{-.2em}{$#2$}\right.}}
\newcommand{\fA}{$\mathfrak{A}$}
\newcommand{\fB}{$\mathfrak{B}$}
\newcommand{\game}[2]{\overline{(#1,#2)}}
\newcommand{\Ind}{$\text{Ind}$}
\newcommand{\im}{\textnormal{im}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\tr}{\text{tr}}
\newcommand{\Tor}{\textnormal{Tor}}
\newcommand{\chr}{\textnormal{char}}
\newcommand{\rank}{\textnormal{rank}}
\newcommand{\Ext}{\textnormal{Ext}}
\newcommand{\dd}{\partial}
 \newcommand{\vol}{\textnormal{vol}}
\renewcommand{\theequation}{\arabic{equation}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\cg}[1]{{\cal #1}}
\newcommand{\Int}{\textnormal{Int}}
\newcommand{\Crit}{\textnormal{Crit}}
\newcommand{\coker}{\textnormal{coker}}
\newcommand{\holim}{\textnormal{holim }}
\newcommand{\hocolim}{\textnormal{hocolim }}
  % prevents \it in theorems
  

%%
%%		          NEWENVIRONMENT DEFINITIONS
%%
%                                                 %	Acknowledgement
\newenvironment{acknowledgement}{%
    \vspace{\medskipamount} 
    \begin{center} 
      \textbf{Acknowledgement} \\[\medskipamount] 
    \end{center}
  }{
    \protect\\ \vspace{\smallskipamount}
  }  
%                                                 %	Claim (unnumbered)
\newenvironment{claim}{%
  \medskip\noindent\textsl{Claim}: \normalfont\upshape}{\medskip}
%                                                 %	Claim (numbered)
\newcounter{acount}\newenvironment{nclaim}{%
    \smallskip\addtocounter{acount}{1}
    \noindent\textsl{Claim \arabic{acount}}: \normalfont\upshape
  }{
    \medskip
  }
%                                                 % Epigraph
\newenvironment{epigraph}{%
    \slshape\small\raggedleft
  }{
    \vspace*{\medskipamount} \\
  }
% Old ssv_artmac example and examples environments ----------
%
% New Examples environment; linked to the example theorem enviroment and counter
% Requires a \firstexample\item followed by \nextexamples\item commands
%                                                  % Examples
%\newcounter{Examples}
%\newcommand{\firstexample}{\renewcommand{\Lbl}{\textsc{Examples: }%
%  \renewcommand{\theexample}{\arabic{example}}
%  \setcounter{Examples}{\theexample}%
%  \addtocounter{Examples}{1}}}
%\newcommand{\nextexample}{\renewcommand{\Lbl}{}}
%\newenvironment{examples}%
%  {\begin{list}{\Lbl\arabic{Examples}) }{\usecounter{Examples}%
%    \setlength{\labelsep}{0pt}\setlength{\leftmargin}{0pt}%
%    \setlength{\labelwidth}{0pt}\setlength{\listparindent}{0.5in}}}%
%  {\setcounter{example}{\theExamples}%
%  \renewcommand{\theexample}{\arabic{example})}\end{list}}   
  % Links Examples counter back to the example counter
% Old ssv_artmac example and examples environments ----------
%
% example and examples environments from ssv_bk -------------
%                                                  % Newest Example Environment
\newcounter{Example}
%-----------------------------------------------
%% Commented out because of problems with LaTeX
%\numberwithin{Example}{section}
%% End commented out because of problems with LaTeX
%-----------------------------------------------
\newenvironment{example}%
    {\renewcommand{\theExample}{\arabic{Example}}\refstepcounter{Example}%
     \begin{list}{}%
        {\usecounter{Examples}%
         \setlength{\labelsep}{0pt}\setlength{\leftmargin}{0pt}%
         \setlength{\labelwidth}{0pt}\setlength{\listparindent}{0.5in}%
        }%
     \item[\normalfont\textsc{Example} \arabic{Example}) ]%
     \renewcommand{\theExample}{\arabic{Example}}%
    }
    {\end{list}}
%                                                  % Newest Examples Environment
\newcounter{Examples}
\newcommand{\firstexample}%
    {\renewcommand{\Lbl}{\textsc{Examples: }}%
     \setcounter{Examples}{\theExample}%
    }
\newcommand{\nextexample}{\renewcommand{\Lbl}{}}
\newenvironment{examples}%
    {\renewcommand{\theExample}{\arabic{Example}}%
     \setcounter{Examples}{\theExample}%
     \refstepcounter{Examples}%
     \begin{list}{\Lbl\arabic{Examples}) }%
        {\usecounter{Examples}%
         \setlength{\labelsep}{0pt}\setlength{\leftmargin}{0pt}%
         \setlength{\labelwidth}{0pt}\setlength{\listparindent}{0.5in}%
        }%
    }%
    {\setcounter{Example}{\theExamples}%
     \renewcommand{\theExample}{\arabic{Example}}\end{list}%
    }   
  % Links Examples counter back to the Example counter
% End of example and examples environments from ssv_bk -------------
%
\newcommand{\Lbl}{}                            % Label identifies exercise type
%                                                 %	Figure captions
\newenvironment{figurecaptions}{%
    \newpage \vspace{\medskipamount}
    \begin{center}
      \textbf{Figure Captions} \\[\medskipamount]
    \end{center}
    \begin{description}
  }{
    \end{description} \vspace{\medskipamount}
  }
%                                                 %	Footnote mylist
\newenvironment{footnotecaptions}{%
    \newpage \vspace{\medskipamount}
    \begin{center}
      \textbf{Footnotes} \\[\medskipamount]
    \end{center}
    \begin{description}
  }{
    \end{description} \vspace{\medskipamount}
  }
%                                                 % mylist environment
\newenvironment{mylist}{%
    \begin{enumerate}
    \renewcommand{\theenumi}{\alph{enumi}}
    \renewcommand{\labelenumi}{{\upshape(\theenumi)}}
  }{
    \end{enumerate}
  }
%                                                 %	Proof
\newenvironment{proof}{%        
    \medskip\noindent\textsc{Proof}:
  }{
    \hfill\qed\medskip
  }
%                                                 %	Proof of Prop. 2
\newenvironment{proofprop2}{%        
    \medskip\noindent\textsc{Proof of Proposition 2}:
  }{
    \hfill\qed\medskip
  }  
%                                                 %	Proof of Prop. 1
\newenvironment{proofprop1}{%        
    \medskip\noindent\textsc{Proof of Proposition 1}:
  }{
    \hfill\qed\medskip
  }  
%                                                 %	Proof of Theorem 1
\newenvironment{proofthm1}{%        
    \medskip\noindent\textsc{Proof of Theorem 1}:
  }{
    \hfill\qed\medskip
  }  
  %                                                 %	Proof of Theorem 5
\newenvironment{proofthm5}{%        
    \medskip\noindent\textsc{Proof of Theorem 5}:
  }{
    \hfill\qed\medskip
  }  
  %                                                 %	Proof of Theorem 8
\newenvironment{proofthm8}{%        
    \medskip\noindent\textsc{Proof of Theorem 8}:
  }{
    \hfill\qed\medskip
  }  
  %                                                 %	Sketch of Proof
\newenvironment{proofsketch}{%        
    \medskip\noindent\textsc{Sketch of Proof}:
  }{
    \hfill\qed\medskip
  }  
    %                                                 %	Proof of Prop. 5
\newenvironment{proofprop5}{%        
    \medskip\noindent\textsc{Proof of Proposition 5}:
  }{
    \hfill\qed\medskip
  }  
    %                                                 %	Proof of Prop. 4
\newenvironment{proofprop4}{%        
    \medskip\noindent\textsc{Proof of Proposition 4}:
  }{
    \hfill\qed\medskip
  }  
  %							%    Proof of Prop. 6
\newenvironment{proofprop6}{%        
    \medskip\noindent\textsc{Proof of Proposition 6}:
  }{
    \hfill\qed\medskip
  }  
%                                                 %	References
\newcounter{bbean}\newenvironment{references}{%
    \begin{list}{%
      [\arabic{bbean}] 
    }{
      \usecounter{bbean} 
    }
  }{
    \end{list}
  }
      %                                                 %	Proof of Lemma 8
\newenvironment{proofoflemma8}{%        
    \medskip\noindent\textsc{Proof of Lemma 8}:
  }{
    \hfill\qed\medskip
    }
      %                                                 %	Proof of Lemma 7
\newenvironment{proofoflemma7}{%        
    \medskip\noindent\textsc{Proof of Lemma 7}:
  }{
    \hfill\qed\medskip
    }
          %                                                 %	Closed-string ms
\newenvironment{closedstringms}{%        
    \medskip\noindent\textsc{Closed-string mirror symmetry}
  }{
    \medskip
    }
%  
  %%%%%%%%
  \newcounter{Remarks}
  \newenvironment{remark}%
    {\renewcommand{\theRemark}{\arabic{Remark}}\refstepcounter{Remark}%
     \begin{list}{}%
        {\usecounter{Remarks}%
         \setlength{\labelsep}{0pt}\setlength{\leftmargin}{0pt}%
         \setlength{\labelwidth}{0pt}\setlength{\listparindent}{0.5in}%
        }%
     \item[\normalfont\textsc{Remark} \arabic{Remark}) ]%
     \renewcommand{\theRemark}{\arabic{Remark}}%
    }
    {\end{list}}
  \newcounter{Remark}
\newcommand{\firstremark}%
    {\renewcommand{\Lbl}{\textsc{Remarks: }}%
     \setcounter{Remarks}{\theRemark}%
    }
\newcommand{\nextremark}{\renewcommand{\Lbl}{}}
\newenvironment{remarks}%
    {\renewcommand{\theRemark}{\arabic{Remark}}%
     \setcounter{Remarks}{\theRemark}%
     \refstepcounter{Remarks}%
     \begin{list}{\Lbl\arabic{Remarks}) }%
        {\usecounter{Remarks}%
         \setlength{\labelsep}{0pt}\setlength{\leftmargin}{0pt}%
         \setlength{\labelwidth}{0pt}\setlength{\listparindent}{0.5in}%
        }%
    }%
    {\setcounter{Remark}{\theRemarks}%
     \renewcommand{\theRemark}{\arabic{Remark}}\end{list}%
    }   
%%%%%%%%                                               %	Remark
%\newenvironment{remark}{%
   % \medskip\noindent\textsc{Remark}:}{\vspace*{\medskipamount}}
%                                                 %	Remarks
%\newenvironment{remarks}{%
  %  \medskip\noindent\textsc{Remarks}:}{\vspace*{\medskipamount}}
%                                                 %	Table Captions
\newenvironment{tablecaptions}{%
    \newpage \vspace{\medskipamount}
    \begin{center}
      \textbf{Table Captions} \\[\medskipamount]
    \end{center}
    \begin{description}
  }{
    \end{description} \vspace{\medskipamount}
  }
%%
%%            NEWTHEOREM DEFINITIONS
%%            Uses Frank Mittlebach's theorem package
%%
% Old definitions -----------------------------------------------
%\theoremstyle{plain}
%\newtheorem{Assertion}{Assertion}     %	Assertion
%\newtheorem{Conjecture}{Conjecture}   %	Conjecture
%\newtheorem{Corollary}{Corollary}     %	Corollary
%{\theorembodyfont{\rmfamily} \newtheorem{Definition}{Definition}}
%{\theorembodyfont{\rmfamily} \newtheorem{Example}{Example}}
%\newtheorem{Fact}{Fact}               %	Fact
%\newtheorem{KeyProperty}{Key Property}       % Key Property
%\newtheorem{Lemma}{Lemma}             %	Lemma
%\newtheorem{MainTheorem}{Main Theorem} % Main Theorem
%\newtheorem{Proposition}{Proposition} %	Proposition
%\newtheorem{Slogan}{Slogan}           % Slogan
%\newtheorem{Theorem}{Theorem}         %	Theorem
%
%\renewcommand{\theAssertion}{\arabic{Assertion}}
%\renewcommand{\theConjecture}{\arabic{Conjecture}}
%\renewcommand{\theCorollary}{\arabic{Corollary}}
%\renewcommand{\theDefinition}{\arabic{Definition}}
%\renewcommand{\theExample}{\arabic{Example}}
%\renewcommand{\theFact}{\arabic{Fact}}
%\renewcommand{\theKeyProperty}{}
%\renewcommand{\theLemma}{\arabic{Lemma}}
%\renewcommand{\theMainTheorem}{}
%\renewcommand{\theProposition}{\arabic{Proposition}}
%\renewcommand{\theSlogan}{\arabic{Slogan}}
%\renewcommand{\theTheorem}{\arabic{Theorem}}
%
%\newtheorem{namedtheorem}{\Lbl}        %   Should be preceded by a \renewcommand{\Lbl}{... theorem name ...} command
%\renewcommand{\thenamedtheorem}{}
%
%\theoremheaderfont{\scshape}
%
%\newenvironment{assertion}%                              % Removes white space
%  {\vspace{-\medskipamount}\begin{Assertion}}{\end{Assertion}}
%\newenvironment{conjecture}%                             % Removes white space
%  {\vspace{-\medskipamount}\begin{Conjecture}}{\end{Conjecture}}
%\newenvironment{corollary}%                              % Removes white space
%  {\vspace{-\medskipamount}\begin{Corollary}}{\end{Corollary}}
%\newenvironment{definition}%                             % Removes white space
%  {\vspace{-\medskipamount}\begin{Definition}}{\end{Definition}}
%\newenvironment{example}%                                % Removes white space
%  {\vspace{-\medskipamount}\begin{Example}}{\end{Example}}
%\newenvironment{fact}%                                   % Removes white space
%  {\vspace{-\medskipamount}\begin{Fact}}{\end{Fact}}
%\newenvironment{keyproperty}%                            % Removes white space
%  {\vspace{-\medskipamount}\begin{KeyProperty}}{\end{KeyProperty}}
%\newenvironment{lemma}%                                  % Removes white space
%  {\vspace{-\medskipamount}\begin{Lemma}}{\end{Lemma}}
%\newenvironment{maintheorem}%                            % Removes white space
%  {\vspace{-\medskipamount}\begin{MainTheorem}}{\end{MainTheorem}}
%\newenvironment{proposition}%                            % Removes white space
%  {\vspace{-\medskipamount}\begin{Proposition}}{\end{Proposition}}
%\newenvironment{slogan}%                                % Removes white space
%  {\vspace{-\medskipamount}\begin{Slogan}}{\end{Slogan}}
%\newenvironment{theorem}%                                % Removes white space
%  {\vspace{-\medskipamount}\begin{Theorem}}{\end{Theorem}}
% Old definitions -----------------------------------------------

% Definitions modified from ssv_bk ------------------------------
\theoremstyle{plain}
\newtheorem{assertion}{Assertion}              %	Assertion
\newtheorem{conjecture}{Conjecture}            %	Conjecture
\newtheorem{corollary}{Corollary}              %	Corollary
{\theorembodyfont{\rmfamily}
\newtheorem{counterexample}{Counterexample}}
{\theorembodyfont{\rmfamily} \newtheorem{definition}{Definition}}
\newtheorem{fact}{Fact}                        %	Fact
\newtheorem{lemma}{Lemma}                      %	Lemma
\newtheorem{proposition}{Proposition}          %	Proposition
\newtheorem{slogan}{Slogan}                    %    Slogan
\newtheorem{theorem}{Theorem}                  %	Theorem
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}

\renewcommand{\theassertion}{\arabic{assertion}}
\renewcommand{\theconjecture}{\arabic{conjecture}}
\renewcommand{\thecorollary}{\arabic{corollary}}
\renewcommand{\thecounterexample}{\arabic{counterexample}}
\renewcommand{\thedefinition}{\arabic{definition}}    
\renewcommand{\thefact}{\arabic{fact}}
\renewcommand{\thelemma}{\arabic{lemma}}
\renewcommand{\theproposition}{\arabic{proposition}}
\renewcommand{\theslogan}{\arabic{slogan}}
\renewcommand{\thetheorem}{\arabic{theorem}}

%  Unnumbered Versions of Newtheorem Environments
\newtheorem{namedtheorem}{\Lbl}                 %   Should be preceded by a \renewcommand{\Lbl}{... theorem name ...} command
\newtheorem{uassertion}{Assertion}              %	Assertion
\newtheorem{uconjecture}{Conjecture}            %	Conjecture
\newtheorem{uconvention}{Convention}            % Convention
\newtheorem{ucorollary}{Corollary}              %	Corollary
{\theorembodyfont{\rmfamily} \newtheorem{ucounterexample}{Counter example}}
{\theorembodyfont{\rmfamily} \newtheorem{udefinition}{Definition}}
{\theorembodyfont{\rmfamily} \newtheorem{uexample}{Example}}
\newtheorem{ufact}{Fact}                        %	Fact
\newtheorem{ukeyproperty}{Key Property}         % Key Property       
\newtheorem{ulemma}{Lemma}                      %	Lemma
\newtheorem{uproposition}{Proposition}          %	Proposition
\newtheorem{uslogan}{Slogan}                    %   Slogan
\newtheorem{utheorem}{Theorem}                  %	Theorem\
\newtheorem{notation}{Notation}

\renewcommand{\thenamedtheorem}{}
\renewcommand{\theuassertion}{}
\renewcommand{\theuconjecture}{}
\renewcommand{\theuconvention}{}
\renewcommand{\theucorollary}{}
\renewcommand{\theucounterexample}{}
\renewcommand{\theudefinition}{}
\renewcommand{\theuexample}{\hspace*{-2pt}:}
\renewcommand{\theufact}{}
\renewcommand{\theukeyproperty}{}
\renewcommand{\theulemma}{}
\renewcommand{\theuproposition}{}
\renewcommand{\theuslogan}{}
\renewcommand{\theutheorem}{}

\theoremheaderfont{\scshape}
%
%		END PREAMBLE
%


